Why Compress What You Can Generate? When GPT-4o Generation Ushers in Image Compression Fields

The rapid development of AIGC foundation models has revolutionized the paradigm of image compression, which paves the way for the abandonment of most pixel-level transform and coding, compelling us to ask: why compress what you can generate if the AIGC foundation model is powerful enough to faithfully generate intricate structure and fine-grained details from nothing more than some compact descriptors, i.e., texts, or cues. Fortunately, recent GPT-4o image generation of OpenAI has achieved impressive cross-modality generation, editing, and design capabilities, which motivates us to answer the above question by exploring its potential in image compression fields. In this work, we investigate two typical compression paradigms: textual coding and multimodal coding (i.e., text + extremely low-resolution image), where all/most pixel-level information is generated instead of compressing via the advanced GPT-4o image generation function. The essential challenge lies in how to maintain semantic and structure consistency during the decoding process. To overcome this, we propose a structure raster-scan prompt engineering mechanism to transform the image into textual space, which is compressed as the condition of GPT-4o image generation. Extensive experiments have shown that the combination of our designed structural raster-scan prompts and GPT-4o's image generation function achieved the impressive performance compared with recent multimodal/generative image compression at ultra-low bitrate, further indicating the potential of AIGC generation in image compression fields.

==> ICCV2025-Author-Kit-Feb/sec/0_abstract.tex <==
\begin{abstract}
\lx{}
The recent breakthroughs in OpenAI’s GPT-4o model have demonstrated impressive image generation and editing capabilities, sparking significant excitement in the community. A natural question arises: can GPT-4o’s advanced image generation capabilities effectively offset the bitrate cost required for image reconstruction? To explore this, we investigate a conditional generation framework that compresses both text and image at the encoder side and feeds them into GPT-4o at the decoder side to reconstruct the final image. Our findings reveal that xxxxxxxxxx.
Experimental results demonstrate that our framework achieves state-of-the-art performance in both consistency and perceptual quality at ultra-low bitrates, without any additional training. 

\end{abstract}





==> ICCV2025-Author-Kit-Feb/sec/1_intro-v1.tex <==
\section{Introduction}
\label{sec:intro}
% 逻辑： 先讲pixel-level coding的问题，比如极低码率下的问题。然后aigc模型的生成能力，分析潜力。点出问题。
% 一些工作已经探索/验证了 生成部分代替压缩 的潜力。最近 gpt4o.....
% 详写方法论，分析结果

Lossy image compression is a cornerstone technology in visual signal communication, significantly reducing bandwidth and storage costs. Currently, lossy image compression methods can be categorized into two types: 1) Traditional coding, where each module is manually designed with multiple modes, and rate-distortion optimization is performed to select the optimal mode~\cite{vvc,bellard_bpg}. 2) Learned image coding, which uses deep neural network modules to implement nonlinear transform coding~\cite{balle2020nonlinear}, achieving end-to-end rate-distortion optimization~\cite{balle2018variational,cheng2020learned,guo2021causal,he2022elic,liu2023learned,minnen2018joint,minnen2020channel,feng2023nvtc,wu2021learned}. Among these methods, both traditional and learned approaches mainly rely on pixel-level transform coding~\cite{goyal2001theoretical} for information transmission. Specifically, they transform pixels into compact representations through a transform module, removing redundancy to lower the bit cost during subsequent entropy coding. 
However, pixel-level coding faces certain issues. These methods primarily focus on local pixel correlations and often lack the ability to capture high-level semantic information. In contrast, human perception tends to prioritize the semantic consistency and texture realism in images, which is difficult to preserve using solely pixel-space transform modules, especially at low bitrates. %This misalignment between pixel-level distortions and human perceptual quality can lead to degraded visual experiences in compressed images.

In recent years, Artificial Intelligence-Generated Content (AIGC) has achieved remarkable progress, particularly in image generation, demonstrating remarkable fidelity and alignment with conditional inputs (\eg, text, sketch maps, reference images). This progress raises a compelling question: why compress what you can generate? If generative models have become sufficiently powerful, could we potentially replace or at least substantially reduce our dependence on conventional pixel-level transform coding? Some previous works~\cite{lei2023text,perco,xue2025dlf,jia2024generative,diffeic,mao2024extreme,xue2024unifying,li2024misc} have offered valuable insights into this question. These studies explored leveraging the priors from pretrained generative models, \eg, Stable Diffusion~\cite{latentdiffusion} and VQ-GAN~\cite{vqgan}, to achieve high-fidelity image compression by transmitting only a small amount of highly compact representations, such as text, sketches, and compact latents. While promising, these approaches often require additional fine-tuning, which compromises the generality and flexibility of the generative model.
The recent breakthroughs in OpenAI’s GPT-4o model~\cite{openai2025gpt4o}, showcasing impressive multimodal image generation and editing capabilities, have generated significant excitement in the community. Motivated by this progress, we aim to explore whether GPT-4o can more effectively address the challenges outlined above without any additional training.

In this paper, we explore two compression paradigms: textual coding and multimodal coding (text combined with an extremely low-resolution image), where all/most pixel-level information is generated rather than compressed, leveraging the advanced image generation capabilities of GPT-4o. 
A major challenge in this generative compression paradigm is how to simultaneously preserve both perceptual quality and consistency with the original image during image generation. To overcome this, we propose a structure raster-scan prompt engineering method. Rather than producing a general caption of the original image, we design a prompt that explicitly guides the multimodal large language model (MLLM) to preserve structural layout and multi-level visual consistency with the original image. 
Specifically, the prompt instructs the MLLM to describe visual elements in a top-to-bottom, left-to-right raster-scan order, preserving the spatial arrangement and relative positioning of objects, which supports geometric consistency and structural integrity. 
In addition, it encourages descriptions that capture distinctive features, object identities, semantic roles, and style properties. By aligning with these multiple levels of visual information, the structured prompt enables more faithful image reconstructions under the generative compression paradigm. We find that this approach effectively maintains the relative positioning between objects, significantly improving the consistency of reconstruction image with the original image.

Building on this strategy, we achieve image compression at bitrates as low as 0.001 bpp while maintaining good perceptual quality and consistency. Experiments demonstrate that our method achieves competitive performance compared to recent generative compression approaches at ultra-low bitrates, even
without any additional training. These results underscore the promising potential of leveraging powerful AIGC foundation models in the field of image compression.






